Contact Mode Guided Motion Planning for Quasidynamic Dexterous Manipulation in 3D

This paper presents Contact Mode Guided Manipulation Planning (CMGMP) for 3D quasistatic and quasidynamic rigid body motion planning in dexterous manipulation. The CMGMP algorithm generates hybrid motion plans including both continuous state transitions and discrete contact mode switches, without the need for pre-specified contact sequences or pre-designed motion primitives. The key idea is to use automatically enumerated contact modes of environment-object contacts to guide the tree expansions during the search. Contact modes automatically synthesize manipulation primitives, while the sampling-based planning framework sequences those primitives into a coherent plan. We test our algorithm on fourteen 3D manipulation tasks, and validate our models by executing some plans open-loop on a real robot-manipulator system

==> sections/0_abstract_old.tex <==
%\sout{Dexterous manipulation in daily human life involves many creative ways of using the contacts between the hand, the object, and the environment.} 
%\sout{Automatic synthesis of such behaviors is computationally difficult because of the hybrid nature of the problem.}


Within the field of robotic manipulation, a central goal is to replicate
the human ability to manipulate any object in any situation using a sequence of
manipulation primitives such as grasping, pushing, inserting, sliding, etc. 
% In addition, robots should also have the ability to generalize across objects and environments. 
Conceptually, each manipulation primitive restricts the object and robot to move on a lower-dimensional manifold defined by the primitive's dynamic equations of motion. Likewise, a manipulation sequence represents a dynamically feasible trajectory that traverses multiple manifolds. % while satisfying boundary constraints between manifolds.
To manipulate any object in any situation, robotic systems must include the ability to automatically synthesize manipulation primitives (manifolds) and sequence those primitives into a coherent plan (find a path across the manifolds).
% are challenging to build due to the non-smooth, non-linear nature of frictional contact dynamics.

%\sout{In this work, we propose a sampling-based planning framework that can quickly and consistently solve 3D %manipulation problems with no pre-specified contact sequence or pre-defined manipulation skill.
%The method uses the guidance of contact modes to explore and cover the vast state space with both continuous and %discrete variables.}

This paper investigates a principled approach for solving dexterous manipulation planning. This approach is based on rapidly-exploring random trees which use contact modes to guide tree expansion along primitive manifolds \cite{cheng2020contact}. 
%The main contribution of this paper is to extend this algorithm from 2D domains to 3D domains. To tackle the increased dimensionality, we devised a method for extending the RRT over a set of locally optimal manipulation primitives which cover the entire action space. Moreover, we addressed numerical errors associated with extending our approach to 3D, and we described a method for generating finger placements on arbitrary 3D meshes. 
This paper extends this algorithm from 2D domains to 3D domains. 
We validated our algorithm on a large collection of simulated 3D manipulation tasks\footnote{The video is available at \url{https://youtu.be/o63dLjIsZmw}. }. These tasks required our algorithm to sequence between 6-42 manipulation primitives (i.e.\! distinct contact modes). We believe this work represents an important step towards robotic manipulation capabilities which generalize across objects and environments.

%These experiments demonstrate the efficacy and efficiency of our algorithmic improvements.

%We demonstrate the efficacy and efficiency of our algorithm in a variety of simulated 3D manipulation tasks. %\sz{a qualitative number might be nice, e.g. by xx\%} 

% Manipulation skills are highly various. Generating such skills is challenging due to the contact-rich nature of manipulation.
% In this paper, we propose a 3D manipulation planning framework that explores the natural connections between contact modes and motion primitives --- they both confine the motions to be on a lower-dimensional manifold with continuous dynamics. Our planner is an RRT-based framework guided by automatically enumerated contact modes which are used to generate ``motion primitives''. The experiments show that this planner requires no predefined manipulation skills, and is general, flexible, and simple to adapt to many different tasks.  

==> sections/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\todo{rewrite, quasi-static and quasi-dynamic}

Manipulation skills used by humans and animals are numerous. For foraging mountain gorillas, \citet{byrne2001manual} document 72 functionally distinct manipulation primitives. With regard to human manipulation, \citet{nakamura2017complexities} find that existing taxonomies cannot categorize many human grasping behaviors in a grocery store. 
Researchers have explored a variety of manipulation skills in depth, including grasping, pushing \cite{mason1986mechanics, lynch1996stable}, tumbling \cite{maeda2004motion}, pivoting \cite{aiyama1993pivot,holladay2015general,hou2018fast}, whole-body manipulation \cite{salisbury1988whole}, extrinsic dexterity \cite{ChavanDafle2014extrinsic}, prehensile pushing \cite{chavan2015prehensile}, regrapsing \citep{tournassoud1987regrasping}, shared grasping \cite{hou2020manipulation}, etc. However, most of these work still requires significant human engineering to design manipulation motions or modeling assumptions to simplify the tasks for the robots, such as pre-defining a sequence of contact modes. 

Automatically generating such dexterous manipulation skills and motions in various scenarios becomes desirable but still challenging. The dexterity in manipulation comes from two resources: the dexterity of robot hands (intrinsic dexterity) and the properties of the environments (extrinsic dexterity). A good general dexterous manipulation motion planner needs to generate strategies that use both intrinsic and extrinsic dexterity cleverly. Moreover, manipulation is contact-rich by nature. Making and breaking contacts bring more complexity into the system by changing its kinematics and dynamics. This hybrid nature makes planning through contacts difficult. This paper aims to move one step closer to general dexterous manipulation planning by considering the dexterity from planning through both the robot hand contacts and environment contacts.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/firstpage_fig.pdf}
    \caption{One example of the problems solved in this paper. The goal is to get the object out of the box while the gaps are too small for both fingers to get in. Our method plans first to push the object on the top to create a wider gap that lets the fingers slide up the object from the side.
    }
    \label{fig:intro}
\end{figure}

The key idea of this paper is to use contact modes as the guidance for dexterous manipulation motion generation. The planner we propose is an RRT~\cite{lavalle1998rapidly} based planner with instantly enumerated contact modes as guidance to extend the tree. We can think of enumerated contact modes as automatically generated ``motion primitives'' as they both define submanifolds of configuration space. Compared with manually designed motion primitives, contact modes can help generate more varied motions, because they can easily capture the discrete changes of the system introduced by contacts, as the set of all feasible contact modes enumerates all possible transitions of the states of contacts in the system. 

Combining contact mode guidance with sampling based planning, our method can perform fast exploration over large continuous and discrete spaces to plan contact-rich motions. One example for peg-out-of-hole/unpacking planning is shown in Figure \ref{fig:intro}. The planner generates the strategy of first pushing the object on the top to create a wider gap that lets the fingers slide up the object from the side, and then form a grasp. 

%The main contribution of this work is to extend 
This work extends our contact-mode guided planner \cite{cheng2020contact} from 2D domains to 3D domains. 
We demonstrate that our 3D planner is a big step closer to general manipulation planning by showing its capability of solving more varied and complicated manipulation tasks that cannot be solved with the 2D formulation. 
The increase in dimensionality creates many non-trivial issues, which we address in this work. The number of contact-modes, though polynomial in the number of contacts $n$, is exponential in the degrees of freedom $d$, which increases from $3$ to $6$ for an object \cite{huang2020efficient}. As forward integrating every primitive is prohibitive, the extend function was modified to integrate a set of locally optimal primitives %whose basins of attraction 
which cover the entire action space. 
When changing from 2D to 3D, the numerical error increased due to multiple reasons outside of our control including increased linearization error and hard-coded collision checking tolerances. To improve numerical robustness, we added a velocity projection step to the forward integration method. Finally, we also describe a method for generating finger placements on arbitrary 3D mesh models, which make our 3D formulation compatible with user-defined manipulator models. 
%With the improved 3D formulation, we demonstrate more varied and more complicated dexterous manipulation tasks that cannot be solved with the 2D formulation.

The rest of this paper is organized as follows. Section \ref{sec:literature} reviews related works. Section \ref{sec:problem_description} provides a mathematical problem description of the 3D manipulation planning problems considered in this paper. Section \ref{sec:model} briefly goes over contact modes in 3D and contact mode constraints for quasi-static manipulation. Section \ref{sec:planner} describes our planning framework. Section \ref{sec:results} presents planning results for general dexterous manipulation and regrasp planning tasks. Section \ref{sec:conclusion} concludes the paper and lists some directions for future work.


==> sections/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

%Page limit:8 not including references

%The dexterity of robotic manipulation could be from many sources. A multi-fingered robotic hand with many degrees of freedom can easily perform in-hand object manipulation by itself \cite{}. On the other hand, extrinsic dexterity also plays a crucial role in manipulation \cite{dafle2014extrinsic}. Many robotic manipulation skills uses environment contacts as one important source of external dexterity. The examples are pushing \cite{mason1986mechanics} \cite{lynch1996stable}, pivoting \cite{aiyama1993pivot}\cite{holladay2015general}\cite{hou2018fast}, tumbling \cite{maeda2004motion}, whole-body manipulation \cite{salisbury1988whole}, prehensile pushing \cite{chavan2015prehensile} and shared grasping \cite{hou2020manipulation}.

\todo{rewrite intro}
\todo{add contributions}
Manipulation skills used by humans and animals are numerous. For foraging mountain gorillas, \citet{byrne2001manual} document 72 functionally distinct manipulation primitives. With regard to human manipulation, \citet{nakamura2017complexities} study human grasping behaviors in a grocery store, while some observed behaviors in \cite{nakamura2017complexities} cannot be categorize by existing taxonomies. 
Researchers have explored a variety of manipulation skills in depth, including grasping, pushing \cite{mason1986mechanics} \cite{lynch1996stable}, tumbling \cite{maeda2004motion}, pivoting \cite{aiyama1993pivot}\cite{holladay2015general}\cite{hou2018fast}, whole-body manipulation \cite{salisbury1988whole}, extrinsic dexterity \cite{ChavanDafle2014extrinsic}, prehensile pushing \cite{chavan2015prehensile}, regrapsing \citep{tournassoud1987regrasping}, shared grasping \cite{hou2020manipulation}, etc. However, most of these work still requires significant human engineering to design manipulation motions or modeling assumptions to simplify the tasks for the robots, such as pre-defining a sequence of contact modes. %\todo{more explicitly: one primitive a paper (normally what people do)? No! We don't want to spend too much effort on designing and analyze them!}
% 
% However, they still cannot cover many dexterous manipulation skills, which are mostly task and environment dependent. 


Automatic planning for dexterous manipulation is challenging. Manipulation is contact-rich by nature. Making and breaking contacts bring more complexity into the system by changing its kinematics and dynamics. Contacts also pose complementary constraints which are difficult to handle in optimization-based methods. Many solutions lie in lower dimensional subspaces of the search space, which have zero possibility of being sampled if no prior knowledge was given.  
%Why planning for it is hard: (1) solutions lower dimensional space of the search spaces (2) discrete changes of kinematics and dynamics caused by contacts (3) contact constraints are more complicated than normal constraints (essentially complementary constraints)
Many previous work avoided such issues by defining high-level motion primitives. A motion primitive confines the search in a subspace of lower dimensions, ensuring solutions to be found. However, it is very hard to come up with a skill library that fulfills the dexterity and flexibility needed in dexterous manipulation. In contrast, contact implicit trajectory optimization (CITO)\cite{posa2014direct}, which is popular in the locomotion community, solves contact sequences and motions together. As most CITO methods rely on nonlinear optimization solvers \cite{manchester2020variational,posa2014direct}, without good initializations, it is often time-consuming or even intractable to find solutions for dexterous manipulation problems with high dimensions of complexity. 
%\todo{mention the state of art of CITO that address this problem, bernado's paper}
Our goal in this paper is to approach 3D dexterous manipulation planning problem in a more global way without any pre-defined manipulation skills.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/firstpage_fig.pdf}
    \caption{One example of the problems solved in this paper. The goal is to get the object out of the box while the gaps are too small for both fingers to get in. Our method plans to first push the object on the top to create a wider gap that let the fingers slide up the object from the side. %The left figure shows the object trajectory. The right figures show the fingertip locations for the major motions.
    }
    \label{fig:intro}
\end{figure}

%\todo{elaborate}
One important property of motion primitives is that they confine the motions to be on a lower dimensional subspace. Interestingly, the set of all kinematically feasible contact modes partition the object configuration space into many subspaces, and each subspace corresponds to a flow (continuous dynamics) of the system. In other words, a contact mode is similar to a motion primitive in the way that they both define a submanifold of object configurations in the original search space. 

The key idea of this paper is to use contact modes as the guidance for dexterous manipulation motion generation.
The planner we propose is a RRT based planner with instantaneously enumerated contact modes as guidance to extend the tree. For one object, 3D contact mode enumeration is fast to compute because its complexity is polynomial to the number of contacts \cite{huang2020efficient}. Here are some intuitions why we use contact modes: 
(1) We can think of enumerated contact modes as automatically generated ``motion primitives''. Compared with manually designed motion primitives, contact modes can help generate more various motions. % and guide the planner to find solutions lie on a lower dimension of the search space.
(2) Discrete changes in kinematics and dynamics of the system can easily be capture by contact modes, as the set of all feasible contact modes enumerates all possible flows of the system.
(3) The set of all feasible contact modes can be seen as the decomposition of linearly approximated contact complementarity constraints \cite{berard2004contact}. Individually solving for each contact mode is like dividing the complementarity constraint into easier sub-problems. Combined with a sampling based planning method, more global solutions can be generated.

Combining contact mode guidance with sampling based planning, our method can perform fast exploration over large continuous and discrete spaces to plan contact-rich motions. This planner can generate solutions that cannot be found by a regular sampling-based planner, and are hard to describe as sequences of manually designed motion primitives. One example for peg-out-of-hole/unpacking planning is shown in Figure \ref{fig:intro}. The planner generates the strategy of first push the object on the top to create a wider gap that let the fingers slide up the object from the side, and then form a grasp. \eric{The main contributions of this paper are hello}

The rest of this paper is organized as follows. Section \ref{sec:literature} reviews related works. Section \ref{sec:problem_description} provides a mathematical problem description of the 3D manipulation planning problems considered in this paper. Section \ref{sec:model} briefly goes over contact modes in 3D and contact mode constraints for quasi-static manipulation. Section \ref{sec:planner} describes our planning framework. Section \ref{sec:results} presents planning results for general dexterous manipulation and regrasp planning tasks. Section \ref{sec:conclusion} concludes the paper and lists some directions for future work.

\todo{we want to say that we can generate contact rich motions very quickly}

==> sections/2_literature.tex <==
\section{Related Work}
\label{sec:literature}
\todo{reduce to half page}
\todo{some background about quasi-static, quasi-dynamic and full dynamic}

\subsection{Manipulation Planning}
%The sources of dexterity in robotic manipulation is various: dexterous hands \cite{jacobsen1986design}, clever motions \cite{tournassoud1987regrasping}, external forces (like gravity) and contacts \cite{dafle2014extrinsic}, etc. Planning for dexterous manipulation is challenging due to the high dimension of the search space, discrete changes in kinematics and dynamics, and the difficulty in modeling the dexterity itself.       

To reduce the complexity of planning contacts, many works predefined high-level motion primitives \cite{toussaint2018differentiable,lozano2014sequential,barry2013hierarchical,woodruff2017planning,berenson2011constrained}. %then it often becomes a Task and Motion Planning problem \cite{lozano2014sequential}. 
Efficient search and optimization algorithms have been developed to solve these motion sequencing/planning problems~\cite{lozano2014sequential,toussaint2018differentiable}. Sampling-based planning methods like CBiRRT~\cite{berenson2009manipulation} and IMACS \cite{kingston2019exploring} are developed to explore the manifolds of a variety of known constraints efficiently. The existence of motion primitives and constrained manifolds essentially reduces the dimensions of search space and confine the search to be on the manifolds defined by these primitives. Most of these methods require predefined states or primitives, which need human labor given a new task or environment. Their solutions are also confined to be the combinatorics of predefined states/primitives. Overall it is impractical to develop a skill library that fulfills the dexterity and flexibility needed in dexterous manipulation. 
In contrast, our work uses contact modes to generate ``motion primitives'' automatically. Automatically enumerated contact modes define constrained manifolds, allowing the planner to find a variety of lower-dimensional solutions that cannot be found by a regular constrained sampling-based planner \cite{berenson2011constrained} which only exploits known constraints.    

Another line of works that reduces the dimensions of search space is utilizing constraints from contacts. Contact formations~\cite{xiao2001automatic} have been explored in~\cite{trinkle1991dexterous,ji2001planning,tang2008automatic,lee2015hierarchical} to plan motions between two rigid bodies. 
They use contact information to decompose the search space into smaller chunks. Search and planning within contact formations are later combined into a complete solution. The applications, however, are still limited to relative motions between two rigid bodies~\cite{tang2008automatic} or in the finer motion range within a robot hand~\cite{trinkle1991dexterous}. \citet{yashima2003randomized} performs in-hand manipulation planning by using predefined contact modes between the hand and the object to capture the discrete changes of kinematics and dynamics. However, they all require to precompute all possible contact formations offline.
%The most similar works to ours are \cite{yashima2003randomized} and \cite{cheng2020contact}.
%The planning framework of \cite{yashima2003randomized} consists of a global planner that samples object configurations by an RRT and a local planner that solves an inverse problem under a specified contact mode to connect two object configurations. 
Our previous work \cite{cheng2020contact} uses RRT and 2D contact mode enumeration to generate dexterous manipulation plans in 2D. However, the manipulation problems it can address are still limited. For example, the previous 2D planner cannot address object reorientation tasks. 3D manipulation problems are much more complicated and harder to solve than 2D ones. This paper extends the models from 2D to 3D, demonstrating much more application scenarios with our new 3D planner. This 3D planner also allows user-defined manipulator models, while our previous 2D planner \cite{cheng2020contact} only considers manipulators as free-moving spheres.


%\subsection{Regrasping planning}
%Dexterity can also be from clever motions. An object reorientation can be achieved by a parallel jaw gripper if regrasp is allowed. 
%Dexterity can also be achieved by a simple gripper that can only perform grasping. Commonly in regrasp planning, stable poses and transition/transfer motions are predefined to perform a graph search \cite{tournassoud1987regrasping,simeon2004manipulation,hou2018fast}. This is similar to defining motion primitives to shrink the search space. In this paper, we will show that our framework is general that it can also be used to perform regrasp planning and requires no predefined stable poses or motion templates.

\subsection{Contact-rich Motion Generation}
%\todo{mention the state of the art of CITO that address this problem, Bernardo's paper}
In recent years, trajectory optimization has been widely adopted to generate contact-rich motion plans. Contact-Invariant Optimization methods~\cite{mordatch2012contact,mordatch2012discovery} produce complex whole-body and manipulation behaviors in simulation, assuming soft contacts which may violate physics laws. Dynamic manipulation planning for rigid bodies are explored in \cite{posa2014direct,Sleiman2019CIO,doshi2020icra,aceituno-cabezas2020rss}. They can plan simple manipulation actions with small numbers of contact transitions, such as pushing, pivoting, and grasping. 
%Using object trajectories as inputs, \cite{aceituno-cabezas2020rss} can plan robot contact trajectories in more complicated environments. 
As most trajectory optimization methods rely on nonlinear optimization solvers, it could be time-consuming and intractable without good initialization, especially when contact schedules are not specified \cite{aceituno-cabezas2020rss,posa2014direct,manchester2020variational}. Some methods formulate the contact-rich problems as combinatorial optimization problems \cite{doshi2019hybrid,valenzuela2016mixed}, which suffer from exponential growth in complexity.  
To our best knowledge, there has not been any trajectory optimization method that can solve the tasks of a similar level of complexity presented in this paper.

%While dynamic analysis introduces more complexity, quasistatic analysis is accurate enough \cite{Mason1986scope,Mason} for more strictly constrained trajectories for low speed and light object tasks. Solutions from our planner can also be used as initial trajectories for dynamic trajectory optimization. 
%\todo{discussion about RL needs to be improved} Reinforcement learning has also shown its effectiveness in generating in-hand manipulation policies \cite{andrychowicz2020learning}. However, such methods require a lot of training and there has not been any application with extra environment contacts involved.


==> sections/6_experiments.tex <==
\section{Results}
\label{sec:results}

\todo{add 3-4 quasi dynamic test cases}
\todo{with robot model}
\todo{do some real robot experiments?}

In this section, we first present the planning results on several representative manipulation tasks. Then we compared our planner with three different planners designed for these tasks based on different philosophies, verified the effectiveness of contact mode guidance.

\subsection{Task Description}
We test our planner with two types of manipulation tasks: general dexterous manipulation tasks and regrasping tasks. 
Both tasks have the same problem description as explained in Section \ref{sec:problem_description}. In the dexterous manipulation tasks, manipulators are two or three free-moving balls. In the regrasping tasks, the manipulator is a free-moving parallel jaw gripper. 

\subsubsection{General Dexterous Manipulation Tasks}

In these tasks, environment collision or manipulator limitations prevent the manipulator from directly picking up the object. Therefore, dexterous manipulation strategies are necessary.
We select ten representative dexterous manipulation tasks that our planner can solve.

Tasks 1-4 are abstracted from manipulation tasks commonly seen in daily life. As shown in Figure \ref{fig:task1-4}, these tasks need dexterous maneuvers because the environment occludes some surface areas of the object. We assume there are three fingers making point contacts.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/task1-4.pdf}
    \includegraphics[width=\columnwidth]{figs/task1-4real.pdf}
    \caption{Objects and environments for Task 1-4. The lower row shows their corresponding real-life scenarios. Task 1: get the first block out of a set of packed blocks. Task 2: retrieve a book from a bookshelf. Task 3: pick up a very thin book from the table \cite{eppner2015exploitation}. Task 4: retrieve a bottle of drink from the fridge full of bottled drinks \cite{nakamura2017complexities}. }
    \label{fig:task1-4}
\end{figure}

\begin{table*}[th]
%\tiny
% \normalsize
\large
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|cccccccccc|ccc}
    \toprule
    \multirow{2}{*}{Task} & \multicolumn{10}{c|}{General Dexterous Manipulation} & \multicolumn{3}{c}{Regrasping} \\
     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13  \\  \midrule

    Success  & 10/10 & 10/10 & 10/10 & 10/10 & 25/30 & 27/30 & 30/30 & 9/10 & 6/10 & 10/10 & 27/30 & 22/30 & 25/30 \\ %\midrule
    
    {Time (second)}  & 5.35 $\pm$ 1.11 & 2.71$\pm$1.29 & 3.91$\pm$1.03 & 1.67 $\pm$ 0.81  & 2.58$\pm$2.57 & 4.2$\pm$2.52 & 1.57$\pm$1.05 & 8.26$\pm$3.9 & 45.47 $\pm$ 10.47 & 0.64$\pm$0.28 & 9.29$\pm$8 & 14.33$\pm$11.86 & 7.58$\pm$6.45\\ %\midrule

    Nodes in Solution   & 9$\pm$2 & 7$\pm$1 & 8$\pm$2 & 6$\pm$1 & 6$\pm$3 & 9$\pm$3 & 10$\pm$5 & 12 $\pm$ 8 & 42$\pm$12 & 7$\pm$3 & 7$\pm$3 & 10$\pm$4 & 16$\pm$11 \\
    
    Nodes in Tree & 55$\pm$16 & 28$\pm$10 & 38$\pm$16 & 27$\pm$20 & 37$\pm$36 & 69$\pm$37 & 60$\pm$39 & 82$\pm$65 & 437$\pm$95 & 18$\pm$8 & 64$\pm$58 & 105$\pm$76 & 79$\pm$55\\
    %\midrule
    %Contact Modes in Path & 3  & 3 & 5 & 5 & 9 & 4.5  & 9.5 \\ 
    \bottomrule
    \end{tabular}}
    \caption{Planning statistics of our planner. A run is successful if a solution can be found within 100 samples (200 samples for Task 9). ``Time'', ``Nodes in Solution'' and ``Nodes in Tree'' are in the format of ``mean'' $\pm$ ``standard deviation'', only taking successful runs into account.}
    \label{tab:experiment}
\end{table*}

\textbf{Task 1: Unpacking/Peg-out-of-hole} 
An object needs to be picked up from a pile of well-packed objects. The hardest part of unpacking well-packed objects is the first object. The small gaps between objects prevent fingers from picking up the first object directly, as shown in the first column, the second row in Figure \ref{fig:task1-4}. 
As can be seen from Figure \ref{fig:intro} and the video, our algorithm consistently plans to push the object to create a wider gap that lets the fingers slide up the object from one side. 

\textbf{Task 2: Bookshelf}  
Similar to task 1, retrieving a book from a bookshelf requires the book to be first slid/pulled out to form a grasp. As shown in Figure \ref{fig:traj} and the video, our algorithm generates strategies of first sliding or pivoting then grasping the book.

 \textbf{Task 3: Pickup a Blade}
Figure \ref{fig:task1-4} shows a daily life scenario where we need to pick up a book or a blade-like object lying on the table but cannot contact its short edges. 
A common strategy used by humans is to slide the object out of the edge of the table to expose its bottom surface for grasping. Our planner also generates similar strategies.

 \textbf{Task 4: Retrieve a Bottle} 
\citet{nakamura2017complexities} document a human grasping behavior called ``simultaneous levering out and grasp formation'', which is observed when a human is trying to retrieve a bottle of drink in a convenience store (Figure \ref{fig:task1-4}). Our planner finds some similar strategies: the manipulator first pivots or pulls out the object to create more space to form a three-finger grasp to pick the bottle up. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/objects3.pdf}
    \caption{Test objects for object reorientation (Task 5-7} and regrasping planning (Task 11-13).
    \label{fig:objects}
\end{figure}

\textbf{Tasks 5-7 are object reorientation tasks}. The objects are \textbf{a cube (Task 5)}, \textbf{a tetromino T-Block (Task 6)}, and \textbf{a hexbolt (Task 7)}, shown in Figure \ref{fig:objects}. The objects cannot be picked up because the number of fingers (2 for Tasks 5-6, 3 for Task 7) is limited; thus, it is hard to form stable grasps (we assume fingers make point contact with the object). The start and goal orientations are randomly sampled from their stable poses on a flat table.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/task8-10.pdf}
    \caption{Start and goal configurations for Tasks 8-10.}
    \label{fig:task8-10}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/paralleljaw.pdf}
    \caption{The simplified parallel jaw gripper used for regrasp planning (Task 11-13).}
    \label{fig:paralleljawgripper}
\end{figure}

Tasks 8-9 test the planner's ability to plan over many contact changes and longer horizons. The number of contacts is two; thus, the object cannot be directly picked up because stable grasps cannot be formed. Environment contacts are heavily relied on as extra supports.

\textbf{Task 8: Push a Cube along a Wall}
The manipulator needs to take a block up to a cliff, as shown in Figure \ref{fig:task8-10}. Only given the start and goal object configuration, our planner successfully generates strategies of push on the floor, push along the cliff, and pivot under gravity.

\textbf{Task 9: An Obstacle Course for a Cube}
The manipulator needs to get the object through several up-and-down stairs. 
This planner can plan different strategies with many contact switches to get through the obstacles using the contacts with the environment as extra supports.

\textbf{Task 10: Object Rolling} shows that our planner also works for rolling contacts. The object is of a peanut shape with a smooth surface (compared to the polyhedron shapes in the previous tasks). Our planner can also plan for rolling contacts, as shown in the video.


\subsubsection{Regrasping Tasks}
Our method can also generate dexterous motions with non-dexterous robot hands. 
In the regrasping tasks, 
the robot hand is a parallel jaw gripper shown in Figure \ref{fig:paralleljawgripper}. The gripper is free to move in the space but only has one degree of freedom for its fingers. We assume each finger makes a patch contact approximated by three point contacts around the fingertip contact point. In this way, stable grasps are possible.
We test \textbf{regrasping planning for a cube (Task 11)}, \textbf{a T-Block (Task 12)}, and \textbf{a hexbolt (Task 13)} shown in Figure \ref{fig:objects}. During each run, the start and goal poses are randomly selected from the object stable poses on a flat table. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/example_trajectory.pdf}
    \caption{Object trajectories by our planner for Task 2, 3, 4 and 8.}
    \label{fig:traj}
\end{figure}

\subsection{Implementation and Planning Results}

We implement the algorithm using C++, with Bullet3 C++ interface \cite{bullet} for collision checking and OpenGL3 for visualization. The code will be released soon.    
%\todo{c++, bullet, what computer, explain the effect inaccuracies of collision detection: slow the process but still works well}
The planner parameters that need adjustments according to tasks are (1) $w_a$ for the distance metrics used in Equation \ref{eqn:se3metric} and \ref{eqn:weightedcost} (2) the translational and rotational distance for \textsc{extend} to move towards $q_{\mathrm{rand}}$. These parameters do not need careful tuning. Being in a reasonable range is enough.

Figure \ref{fig:traj} visualizes the object trajectories in some select solutions for Task 2,3,4 and 8. Please check the supplementary video for more complete solution visualization. Table \ref{tab:experiment} shows the planning statistics provided by a computer with the Intel Core i9-10900K 3.70GHz CPU. In general, our planner can generate most contact-rich motion plans in a few seconds, except for Task 9, which is of a longer horizon. The number of nodes in the tree is small, indicating that the exploration is efficient. 


%The following is some general discussions about this planner's performance. About 90\% of the planning time (varying across tasks) is spent on the function \textsc{forward-integrate}, a numerical integration process that can be improved in many ways. Another way to largely improve the planning time is that Line 7-9 in Algorithm \ref{alg:rrt} can be easily paralleled. \todo{try to parallel?}  There is an issue about collision checking with line and face contacts. A lot of time the collision checking returns multiple contacts in the interior of a line contact or a face contact, and they are not consistent across time-steps. This causes a break in our forward integration, since it thinks that there are contacts making and breaking. Although our planner is still able to generate reasonable solutions under these circumstances, it is slowed down. A fix to this issue will greatly improve the planning performance on general objects.

\subsection{Comparison and Analysis}

\begin{table}[]

    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lc|ccc}
    \toprule
    \multicolumn{2}{c|}{Task} & 1 & 6 & 8\\  \midrule
    \multirow{4}{*}{Success} & Ours & 10/10 & 27/30 & 10/10 \\ %\midrule
    & \textit{ExtendAll}  & 10/10 & 22/30 & 9/10\\ 
    & \textit{ExtendOne}  & 10/10 & 17/30 & 3/10 \\
    & \textit{ProjectConfig} & 4/10 & 16/30 & 8/10  \\\midrule
    \multirow{4}{*}{Time (second)}  & Ours & 5.35$\pm$1.11 & 4.2$\pm$2.52 & 8.26$\pm$3.9 \\ %\midrule
    & \textit{ExtendAll} & 64.4$\pm$8.5 & 83.0$\pm$22.9 & 26.7$\pm$18.7 \\
    & \textit{ExtendOne} & 123$\pm$164 & 31.8$\pm$16.9 & 149$\pm$110\\
    & \textit{ProjectConfig}  & 2.7$\pm$4.8 & 26.7$\pm$12.9 & 8.9$\pm$2.2 \\ \midrule
    \multirow{4}{*}{Nodes in Solution} & Ours & 9$\pm$2 & 9$\pm$3 & 12$\pm$8 \\ %\midrule
    & \textit{ExtendAll} & 5$\pm$1 & 6$\pm$2 & 12$\pm$2  \\
    & \textit{ExtendOne} & 8$\pm$1 & 9$\pm$5 & 17$\pm$3  \\
    & \textit{ProjectConfig} & 9$\pm$1 & 30$\pm$38 & 30$\pm$10 \\\midrule
    \multirow{4}{*}{Nodes in Tree} & Ours & 55$\pm$16 & 69$\pm$37 & 82$\pm$65 \\ %\midrule
    & \textit{ExtendAll} & 211$\pm$94 & 328$\pm$232 & 693$\pm$73  \\
    & \textit{ExtendOne} & 12$\pm$4 & 14$\pm$11 & 27$\pm$11 \\
    & \textit{ProjectConfig} & 11$\pm$3 & 62$\pm$87 & 45$\pm$23 \\
    \bottomrule
    \end{tabular}}
    \caption{Comparison between our planner and planner \textit{ExtendAll}, \textit{ExtendOne}, and \textit{ProjectConfig}. A run is successful if a solution can be found in 50 samples for our planner, planner \textit{ExtendAll} and planner \textit{ExtendOne}, in 1000 samples for planner \textit{ProjectConfig}.}
    \label{tab:comparison}

\end{table}

We designed three planners to compare with our proposed planner. Table \ref{tab:comparison} shows the planning statistics. Each planner has a different underlying philosophy. We compare these underlying ideas and provide some analysis about manipulation problems.

Planner \textit{ExtendAll} has the same framework as our planner. Instead of extending the best SS mode of every CS mode, planner \textit{ExtendAll} extends all contact modes. It uses contact mode guidance in a simple way that it just uses all modes as ``motion primitives''. In contrast, our planner further uses the information about contacts --- thinking of all feasible CS modes as the enumeration of possible transitions of current contact formation to its adjacent contact formations. Contact formations naturally decompose the search space into small chunks \cite{trinkle1991dexterous} of different dimensions. To explore each chunk, we only need to iterate through all CS modes and find the best motion. As a result, while planner \textit{ExtendAll} has a similar success rate and even smaller solution size than our planner, it spends significant time generating a solution due to the large number of 3D contact modes. It is also unnecessary and impractical to spend the planning time on numerical integration of repeatedly generating similar motions under the same CS mode.

Planner \textit{ExtendOne} only extends one best contact mode among all modes. It is similar to solving the optimization problem of getting close to the goal configuration with linear complementary constraints --- there is a one-to-one correspondence between contact modes and the complementary cones of LCP.  
However, its planning time is even longer, because it ignores useful and stable motions on other manifolds that may take some detours --- it has no idea of ``motion primitives''. 

Planner \textit{ProjectConfig} is similar to CBiRRT \cite{berenson2009manipulation}. %It projects object configurations onto contact manifolds but has no idea what a contact mode is. In its \textsc{Extend} function, it linearly interpolates a path between $x_{near}$ and $x_{rand}$. For every configuration on the path, it projects the configuration onto the contact manifold if penetration detected, 
In its \textsc{Extend} function, it projects the object configuration onto the contact manifold if penetration detected, and checks for force balance under current contacts. 
This planner uses the concepts of projecting the configuration onto the constraint manifold in \cite{berenson2011constrained}. The results show that this concept effective and useful. But it lacks the concept of contact modes, the motions it generates are even less realistic than quasistatic manipulation (because it can only assume every contact is sticking). Most importantly, it cannot find any solution that lies on any manifold of lower dimensions than the contact manifold. For example, theoretically, it cannot generate a two-contact-sticking rotation motion for an object on a flat table. As a comparison, our planner is also a constrained sampling-based planner with the critical improvement of using contact modes to define and generate constrained manifolds.

%In a word, the above comparison shows the effectiveness of contact mode guidance. Contact modes help guide more realistic motion generation on lower-dimensional manifolds that are hard to be found otherwise. 


